The Carina Project. VIII. The {\alpha}-element abundances

We have performed a new abundance analysis of Carina Red Giant (RG) stars from spectroscopic data collected with UVES (high resolution) and FLAMES/GIRAFFE (high and medium resolution) at ESO/VLT. The former sample includes 44 RGs, while the latter consists of 65 (high) and ~800 (medium resolution) RGs, covering a significant fraction of the galaxy's RG branch (RGB), and red clump stars. To improve the abundance analysis at the faint magnitude limit, the FLAMES/GIRAFFE data were divided into ten surface gravity and effective temperature bins. The spectra of the stars belonging to the same gravity/temperature bin were stacked. This approach allowed us to increase by at least a factor of five the signal-to-noise ratio in the faint limit (V>20.5mag). We took advantage of the new photometry index cU,B,I introduced by Monelli et al. (2014), as an age and probably a metallicity indicator, to split stars along the RGB. These two stellar populations display distinct [Fe/H] and [Mg/H] distributions: their mean Fe abundances are -2.15$\pm$0.06dex (sig=0.28), and -1.75$\pm$0.03dex (sig=0.21), respectively. The two iron distributions differ at the 75% level. This supports preliminary results by Lemasle et al. (2012) and by Monelli et al. (2014). Moreover, we found that the old and intermediate-age stellar populations have mean [Mg/H] abundances of -1.91$\pm$0.05dex (sig=0.22) and -1.35$\pm$0.03dex (sig=0.22); these differ at the 83% level. Carina's {\alpha}-element abundances agree, within 1sigma, with similar abundances for field Halo stars and for cluster (Galactic, Magellanic) stars. The same outcome applies to nearby dwarf spheroidals and ultra-faint dwarf galaxies, in the iron range covered by Carina stars. Finally, we found evidence of a clear correlation between Na and O abundances, thus suggesting that Carina's chemical enrichment history is quite different than in the globular clusters.

==> tab_linelist.tex <==
\begin{table}
\footnotesize
\caption{Atomic Data}
\label{tab_linelist}
\centering
\begin{tabular}{lcccc}
\hline\hline
%%
 {$\lambda$ (\AA)}&
 {Elem.}&
 {$\chi$ (eV)}&
 {$\log gf$}&
 {Damp.}\\
\hline
\multicolumn{5}{l}{\bf GIRAFFE HR10}\\
5336.770 & Ti2 &     1.58 &    -1.59 &    -7.95\\
5339.929 & Fe1 &     3.26 &    -0.64 &    -7.22\\
5341.023 & Fe1 &     1.60 &    -1.95 &    -7.68\\
\dots & \dots & \dots & \dots & \dots \\
\hline
\multicolumn{5}{l}{\bf GIRAFFE HR13}\\
\dots & \dots & \dots & \dots & \dots \\
\hline
\multicolumn{5}{l}{\bf GIRAFFE HR14}\\
\dots & \dots & \dots & \dots & \dots \\
\hline
\multicolumn{5}{l}{\bf GIRAFFE LR08}\\
\dots & \dots & \dots & \dots & \dots \\
\hline
\multicolumn{5}{l}{\bf UVES}\\
\dots & \dots & \dots & \dots & \dots \\
\hline
\end{tabular}
\tablefoot{This table is available entirety in a machine-readable form in the 
online journal. A portion is shown here for guidance regarding its form and content.}
\end{table}


==> tab_means.tex <==
%\begin{sidewaystable*}
\begin{table*}
\footnotesize
\caption{Mean abundances and dispersions for individual sub-samples.}
\label{tab_means}
\centering
\begin{tabular}{c cccc}
\hline\hline
%%
 {Popul.}&
 {UVES} & {GHR} & {GMR} & {ALL}\\
 {}&
 {indiv./EW} & {stack./EW} & {stack./SYNT}\\
 \hline
\multicolumn{4}{c}{\bf\feih} \\
 old & -2.31$\pm$0.25[10] & -2.19$\pm$0.27[4] & -1.93$\pm$0.16[9]\\
  int & -1.81$\pm$0.18[34] & -1.69$\pm$0.18[4] & -1.54$\pm$0.23[10]\\
\hline
\multicolumn{4}{c}{\bf\oife} \\
 old & \dots & \dots & \dots \\
  int & 0.55$\pm$0.09[6] & \dots & \dots\\
\hline
\multicolumn{4}{c}{\bf\naife} \\
 old & \dots & \dots & \dots \\
  int & 0.32$\pm$0.31[3] & \dots & \dots\\
\hline
\multicolumn{4}{c}{\bf\mgife}\\ 
 old & 0.28$\pm$0.08[3] & 0.39$\pm$0.19[4] & 0.16$\pm$0.17[7] \\
  int & 0.48$\pm$0.18[22] & 0.35$\pm$0.11[4] & 0.29$\pm$0.16[10]\\
\hline
\multicolumn{4}{c}{\bf\siife}\\
 old & \dots & \dots & \dots \\
  int & 0.49$\pm$0.17[9] & \dots & \dots\\
\hline
\multicolumn{4}{c}{\bf\caife}\\
old & 0.17$\pm$0.40[10] & 0.22$\pm$0.09[4] & \dots\\
 int & 0.28$\pm$0.13[34] & 0.25$\pm$0.05[4] & \dots\\
\hline
\multicolumn{4}{c}{\bf\tiiife}\\
 old & 0.40$\pm$0.37[9] & 0.38$\pm$0.18[4] & \dots\\
  int & 0.25$\pm$0.29[32] & 0.51$\pm$0.15[4] & \dots\\

\hline
\multicolumn{4}{c}{\bf[\mgi+\cai/2Fe]}\\
 old & 0.25$\pm$0.40[10] & 0.31$\pm$0.12[4] & \dots \\
  int & 0.36$\pm$0.15[32] & 0.30$\pm$0.08[4] & \dots\\
\hline
\multicolumn{4}{c}{\bf$\mathbf\alpha$-el.=[\mgi+\cai+\tiii/3Fe]} \\
 old & 0.34$\pm$0.30[9] & 0.33$\pm$0.12[4] & \dots \\
  int & 0.32$\pm$0.17[32] & 0.37$\pm$0.05[4] & \dots\\
\hline 
\end{tabular}

\end{table*}
%\end{sidewaystable*}

